Unsupervised Risk Estimation Using Only Conditional Independence Structure

We show how to estimate a model's test error from unlabeled data, on distributions very different from the training distribution, while assuming only that certain conditional independencies are preserved between train and test. We do not need to assume that the optimal predictor is the same between train and test, or that the true distribution lies in any parametric family. We can also efficiently differentiate the error estimate to perform unsupervised discriminative learning. Our technical tool is the method of moments, which allows us to exploit conditional independencies in the absence of a fully-specified model. Our framework encompasses a large family of losses including the log and exponential loss, and extends to structured output settings such as hidden Markov models.

==> learning-algorithm.tex <==
\begin{algorithm}[t]
\caption{Algorithm for computing the gradient of $\riski$.}
\label{alg:gradient}
\scalebox{0.952}{\begin{minipage}{1.05\columnwidth}
  \begin{algorithmic}
    \STATE \textbf{Input:} initial parameters $\theta_0 \in \bR^d$, samples $x^{(1:m)} \sim p^*$.
    \STATE Define $h_v(x,u) \in \bR^{2k}$ as 
           \vskip -0.23in
           \begin{equation*}h_v(x,u) = [f_{v}(\theta_0; x_v,j)\,\,\,\, u^{\top}\nabla_{\theta} f_{v}(\theta_0; x_v,j)/B]_{j=1}^k\end{equation*}
    \STATE \vskip -0.2in \FOR{$t = 1$ to $T = \frac{75d\log(2d/\delta)}{\epsilon^2}$}
    \STATE Sample $u_t$ uniformly from $\{\pm 1\}^d$.
    \STATE Using $x^{(1:m)}$, estimate the moments 
    \vskip -0.27in
\begin{align*}&\bE[h_v(x,u_t)], \bE[h_{v_1}(x,u_t) \otimes h_{v_2}(x,u_t)], \text{ and }\\ &\bE[h_1(x,u_t) \otimes h_2(x,u_t) \otimes h_3(x,u_t)].\end{align*}
    \vskip -0.15in
    \STATE \vskip -0.08in Use tensor decomposition to compute $\hat{\pi}_{j,t} \approx \pi_j$, 
           $\hat{\mu}_{j,t} \approx \sum_v \mu_{j,v}$, and 
           $\hat{g}_{j,t} \approx \sum_v \bE[u_t^{\top}\nabla_{\theta} f_v(\theta_0; x_v,j) \mid j]$.
           % JS: I agree but don't see a nice way to fix, so de-prioritizing for now
           %\pl{seems like you should actually define $\hat g$ in terms of $\hat\mu$,
           %since technically tensor decomposition doesn't give you $\hat g$}
    \STATE Permute the rows of $\hat{\mu}_{j,t}$ (and simultaneously $\hat{g}_{j,t}$) such that $\sum_j \hat{\pi}_{j,t}(\hat{\mu}_{j,t})_j$ is maximized.
    \ENDFOR
    \STATE Output $\hat{g} = \frac{1}{T} \sum_{t=1}^T u_t \sum_{j=1}^k \hat{\pi}_{j,t} \hat{g}_{j,t}$.
  \end{algorithmic}
\end{minipage}}
\end{algorithm}

